Enabling Atomic Durability for Persistent Memory with Transiently Persistent CPU Cache

Persistent memory (pmem) products bring the persistence domain up to the memory level. Intel recently introduced the eADR feature that guarantees to flush data buffered in CPU cache to pmem on a power outage, thereby making the CPU cache a transient persistence domain. Researchers have explored how to enable the atomic durability for applications' in-pmem data. In this paper, we exploit the eADR-supported CPU cache to do so. A modified cache line, until written back to pmem, is a natural redo log copy of the in-pmem data. However, a write-back due to cache replacement or eADR on a crash overwrites the original copy. We accordingly develop Hercules, a hardware logging design for the transaction-level atomic durability, with supportive components installed in CPU cache, memory controller (MC), and pmem. When a transaction commits, Hercules commits on-chip its data staying in cache lines. For cache lines evicted before the commit, Hercules asks the MC to redirect and persist them into in-pmem log entries and commits them off-chip upon committing the transaction. Hercules lazily conducts pmem writes only for cache replacements at runtime. On a crash, Hercules saves metadata and data for active transactions into pmem for recovery. Experiments show that, by using CPU cache for both buffering and logging, Hercules yields much higher throughput and incurs significantly fewer pmem writes than state-of-the-art designs.

==> ad5.tex <==
\subsection{Atomic Durability}\label{sec:bg-ad}

 
The atomic durability, or failure-atomic durability, refers to the
crash consistency of modifying in-pmem data in case of a
crash. 
The insertion with an in-pmem sorted array mentioned in Section~\ref{sec:intro}
is a typical {transaction} programmers would 
define with their desired semantics.  
A transaction must be done 
in an atomic (all-or-nothing) fashion.  
Otherwise, a half-done change may 
leave data in ambiguity or uncertainty
after a crash.
 
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\columnwidth]{./pic/bg2.pdf}
		\vspace{-1ex}
		\caption{{An Illustration of Persistence Domains Explored in Prior Works and This Paper}} \label{fig:cache-persistency}
	\end{center}
	\vspace{-5ex}
\end{figure} 
 
 
\subsubsection{Software Solution} 
\ \newline
\indent Modern 64-bit CPUs allow an atomic write of up to  
8 bytes.
Programmers bundle multiple data operations 
for a task  
in one transaction and seek software or hardware solutions.
Software logging is a common technique. Programmers  
explicitly record original (resp. modified) data in an undo (resp. redo) log.
However, 
software logging is not effectual  
with several factors.
Firstly, logging incurs double writes  
due to writing both log and data copies~\cite{txm:Kiln:MICRO13,pmem:UBJ:FAST-2013,txm:ReDU:Micro-2018,arch:PS-ORAM:ISCA-2022}.
Double  
writes 
jeopardize performance and impair lifetime for NVM technologies 
that
have limited write endurance~\cite{pmem:PCM:Micro-2009,arch:endurance:ASPLOS-2010,arch:PCM-refresh:IEEE-Micro-2011,arch:SD-PCM:ASPLOS-2015,arch:ReRAM-endurance:TACO-2018,pmem:FlatStore:ASPLOS-2020,arch:PCM:HPCA-2022}.
Secondly, logging demands extra instruction to be executed.
Log and data copies also consume more
architectural resources.  
For example,
they need double locations in pmem.
If programmers use CPU cache to buffer them, they take double cache lines.
Thirdly, the ordering of writing log copies prior to data must 
be retained by using memory fences,
the cost of which, albeit the presence of eADR, 
is essential and
substantial~\cite{pmem:orderless:ICCD-2014,txm:transaction-cache:DAC17,pmem:fence-less:Micro-2020}.





\subsubsection{Hardware Designs}\label{sec:ad:hardware}
\ \newline
\indent  The essence of gaining atomic durability 
is to make a backup copy before  
modifying data in place.
In order
to back up data,
state-of-the-art hardware designs explore different persistence domains, which categorize
them into three classes.
 


 
\textbf{Persistent CPU cache.}\hspace{0.5ex}
{As shown in~\autoref{fig:cache-persistency},
Kiln works with a persistent  
last-level cache (LLC)}~\cite{txm:Kiln:MICRO13}.
The persistence domain covers LLC and pmem. 
Kiln manages redo log copies in LLC to back up
in-pmem data.
Later,
Lai et al.~\cite{txm:transaction-cache:DAC17} employed a side-path persistent
transaction cache (TC) along L1 
cache in each CPU core. TC is similar to the 
persistent buffers used in other works~\cite{arch:BBB:HPCA-2021,arch:TSOPER:HPCA-2021}.
Modified cache lines of a transaction
are first-in-first-out (FIFO)
put in the TC  
and serially written 
to pmem 
on committing a transaction.
 

 
\textbf{Pmem.} {A few hardware designs were built on
a pmem-only persistence domain.}
Doshi et al.~\cite{txm:backend:HPCA-2016} proposed to use a victim cache
to hold evicted cache lines that would be 
subsequently written to an in-pmem redo log. 
These cache lines
are eventually 
written to their home addresses
by copying log entries via non-temporal stores.
Similarly, Jeong et al.~\cite{txm:ReDU:Micro-2018} proposed ReDU that utilizes
a DRAM cache to hold evicted cache lines from the LLC.
ReDU directly
writes modified data from DRAM cache
to home addresses, as it
installs a log buffer alongside L1 cache to collect 
and write the in-pmem redo log.

Cai et al.~\cite{txm:HOOP:ISCA20}
designed HOOP  
with a physical-to-physical address indirection layer in the MC, which
helps it
write modified data to a different pmem address for backup
and later  
move data to home addresses.  
Joshi et al.~\cite{txm:ATOM:HPCA-2017} noted that 
the MC loads a cache line for a write request 
and proposed ATOM to 
write the loaded copy to an in-pmem undo log in a parallelized manner.
Nguyen and Wentzlaff~\cite{txm:PiCL:MICRO18} proposed PiCL that also uses the idea of
undo logging with  
an on-chip log buffer. 
PiCL makes a trade-off between performance and durability
by snapshotting and saving data
in an epoch-based periodical checkpointing manner~\cite{txm:checkpoint-SST-RAM:ICCAD-2014}.
Ogleari et al.~\cite{txm:Steal-but-No-Force:HPCA18} and Wei et al.~\cite{txm:MorLog:ISCA-2020}
both chose the undo+redo logging approach.  
Ogleari et al. captured data's 
redo and undo log copies from the in-flight write operation and the write-allocated 
cache line, respectively.
They also used a force write-back (FWB) mechanism to control pmem writes.
Wei et al. studied data encoding with hardware  
logging
so as to only record necessary changes for a transaction's data, thereby reducing pmem writes.
Both designs 
add on-chip undo and redo log buffers.
 
\begin{figure*}[t]
	\begin{subfigure}{0.193\textwidth}
		\includegraphics[width=\textwidth]{pic/mot/mota-woeadr2.pdf}
		\caption{Sample Code on Logging~\cite{arch:blurred-persist:TOS-2016,txm:transaction-cache:DAC17,txm:ATOM:HPCA-2017,txm:Proteus:MICRO17,txm:Steal-but-No-Force:HPCA18,txm:ReDU:Micro-2018}}
		\label{fig:mot:code}
	\end{subfigure}	
	\hfill
	\begin{subfigure}{0.193\textwidth}
		\includegraphics[width=\textwidth,page=1]{pic/mot/mot.pdf}
		\caption{Throughput}
		\label{fig:mot:thruput}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.193\textwidth}
		\includegraphics[width=\textwidth,page=2]{pic/mot/mot.pdf}
		\caption{Pmem Writes}
		\label{fig:mot:writes}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.193\textwidth}
		\includegraphics[width=\textwidth,page=3]{pic/mot/mot.pdf}
		\caption{Cache Accesses}
		\label{fig:mot:cache}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.193\textwidth}
		\includegraphics[width=\textwidth,page=1]{pic/mot/mot4.pdf}
		\caption{Executed Instructions and CPU Clock Cycles}
		\label{fig:mot:inst}
	\end{subfigure}
	\caption{A Study on Software Logging Logging with/without eADR and State-of-the-art Hardware Designs for Atomic Durability}
	\vspace{-3ex}
\end{figure*}


 
\textbf{ADR-supported transient persistence domain.}\hspace{0.5ex}
{The ADR places 
the WPQ of MC in the transient persistence domain}.  
Shin et al.~\cite{txm:Proteus:MICRO17} designed Proteus
 that  
considers the  
WPQ to keep log copies.
When a transaction commits, Proteus discards relevant log copies in the WPQ
and hence reduces pmem writes. 
Gupta et al.~\cite{txm:LAD:MICRO19} proposed LAD that also
leverages the ADR-supported 
MC as a staging buffer
to accumulate data updates before committing a transaction.
Whereas,  
for Proteus and LAD,
the limited capability of WPQ  
entails a high likelihood 
of falling back to the use of an in-pmem log.  
  

==> eval6.tex <==
\section{Evaluation}\label{sec:eval}


\subsection{Evaluation Setup}\label{subsec:setup}

We have implemented and evaluated \Attend 
%and the other hardware transactional memory (HTM) variants on 
%in the gem5 simulator
with gem5 %~\cite{sim:gem5}
in the syscall emulation (SE) mode and `classic caches' model. 
\autoref{tab:config} captures the settings of CPU with three-level caches
that generally align 
with
%As captured in~\autoref{tab:config}, 
%we configure a multi-core out-of-order CPU 
%with eADR-supported three-level caches in accordance with 
previous works~\cite{txm:Kiln:MICRO13,txm:transaction-cache:DAC17,txm:Proteus:MICRO17,txm:HOOP:ISCA20,txm:PiCL:MICRO18,txm:ReDU:Micro-2018}.
% ARM CPU instead of using x86 ISA because of its synchronization issue in the multi-threading. We found that it is unable to run the multi-threading with locking workloads with x86 architecture in either SE mode or full system (FS) mode. 
%Moreover, it is necessary to gather more realistic results with multi-threading workloads, and we believe that the support of pmem and eADR can be available in the ARM architecture in the future. 
We set the write/read latencies of pmem as 100ns/150ns
%, which is higher than the write latency of 100ns,
according to a recent study%of Intel Optane DC persistent memory
~\cite{pmem:Optane-study:FAST-2020}. 
%%%%More than that, we set the read/write buffer size to 64 based on the previous pmem research\todo{cite}.
%In 
%To reduce the cache extension overhead, we maintain a ratio of transactional cache lines, and we set the optimal (100\%) in the following evaluation. 
%By default, we install TransTags for all cache lines per set and have a discussion on the ratio of TransTags in Section~\ref{sec:ratio-eval}.
We set the ratios of TransTag to be 100\%/50\%/25\% for L1D/L2/L3, respectively.
%As the capacity is valuable in the L1D cache, 
Particularly for fairness, %as shown in~\autoref{tab:config},
%%%regarding the valuable space of L1D cache,
we %comparatively 
reduce 
the L1D size of \Attend 
from 32KB to 30KB 
by removing some cache lines to 
counterbalance the spatial cost of TransTags
and add 25.0\% more tag latency as the temporal cost
for cache line access involving a TransTag. 
%counteract tag overhead instead of reducing the ratio of transactional cache lines in the L1d cache. 
We set a commit latency in ten cycles
to find and toggle {\tt TxState}s of %involved %
transactional 
cache lines when a transaction commits and
%We 
have a discussion on
the impact of this latency in Section~\ref{sec:scan-eval}.
%We will configure the different ratios of transactional cache lines and cache scan overhead to identify the efficiency and rationality of our proposal. 
%In addition, we 
We also
set ten cycles for searching the eWPQ %entries %look up the address mapping in the premature flush buffer 
to check if a cache line has been prematurely flushed or not. % to pmem.
%if an uncommitted cache line is evicted to the pmem.

\begin{table}[t]
	\centering
	\caption{System Configuration}\label{tab:config}
	\vspace{-1ex}	
	\resizebox{\linewidth}{!}{
		\begin{tabular}{|l|l|l|}
			\hline
			Component & Setting & Remarks \\ \hline\hline
			Processor & 3GHz, out-of-order, 8 cores & \multirow{8}{*}{Generic} \\ \cline{1-2}
			L1I Cache & 32KB, 4-way, 2-cycle latency &\\ \cline{1-2}
			L1D Cache & 32KB, 4-way, 2-cycle latency&\\ \cline{1-2}
			L2 Cache & 256KB, 8-way, 8-cycle latency&\\ \cline{1-2} % inclusive
			LLC & 16MB, 16-way, 30-cycle latency&\\  \cline{1-2}
			\multirow{2}{*}{pmem} & Read/Write latency=150ns/100ns,  capacity=512GB, & \\ & Single Channel, read/write buffer size=64&\\  \hline
			Smaller L1D Cache & 30KB, 4-way, 2/2 cycles read/write latencies& \Attend only \\  \hline			
			Side-path TC&4KB, FIFO, 40/50 cycles read/write latencies& TC~\cite{txm:transaction-cache:DAC17} only \\ \hline
			STT-RAM LLC & 64MB, 16-way, 40/50 cycles read/write latencies& Kiln~\cite{txm:Kiln:MICRO13} only \\ \hline
			%			Large SRAM LLC &64MB, 16-way, 30 cycles latency&OPT\_64 only\\ \hline
		\end{tabular}
	}
	\vspace{-2ex}
\end{table}


\begin{comment}
	
	In~\autoref{tab:config}, 
	the STT-RAM LLC 
	%For the STT-RAM cache, which 
	is used by Kiln. We configure a larger capacity and longer access latency in line with 
	the physical characteristics of STT-RAM, e.g., higher density and slower access speed~\cite{arch:STT-RAM:Micro-2011,txm:Kiln:MICRO13}.
	%in line with the original literature.
	The side-path STT-RAM cache for the design of TC is set in 4KB regarding
	%in line
	%with regard to 
	its literature~\cite{txm:transaction-cache:DAC17}. 
	%compared with the regular cache based on their original paper. 
	%The STT-RAM cache has 64MB capacity in Kiln and 4KB in TC. 
\end{comment}


\begin{table}[b]
	\centering
	\caption{Benchmarks Used in the Evaluation}\label{tab:benchmark}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{|l|l|l|}
			\hline
			Category& Benchmark& Remarks \\ \hline\hline
			\multirow{7}{*}{Micro-benchmarks}
			& Array Swap & Swaps two elements in an array  \\\cline{2-3}
			& Binary Heap & Inserts/deletes entries in a dary heap  \\\cline{2-3}
			& B+-Tree & Inserts/deletes KV pairs in B+-tree \\\cline{2-3}
			& Hash Table & Inserts/deletes entries in a hash table \\\cline{2-3}
			& Linked List & Inserts/deletes entries in a linked list \\\cline{2-3}
			& RB-Tree & Inserts/deletes entries in a RB-Tree \\\cline{2-3}
			& SDG & Inserts/deletes edges in a scalable large graph \\\hline
			\multirow{2}{*}{Macro-benchmarks}
			& TPC-C & OLTP workload (New-order transactions)  \\\cline{2-3}
			& YCSB & 80\%/20\% of write/read \\\hline			
		\end{tabular}
	}
\end{table}

\autoref{tab:benchmark} summarizes the benchmarks we use
for evaluation. 
%Micro-benchmarks are data structures widely used in applications
We consider widely-used data structures as micro-benchmarks
%by following 
like previous works~\cite{txm:Kiln:MICRO13,txm:HOOP:ISCA20,txm:ATOM:HPCA-2017,txm:Steal-but-No-Force:HPCA18}.
We utilized YCSB and TPC-C from WHISPER
as macro-benchmarks~\cite{NVM:recovery:SIGMOD-2015,arch:Whisper:ASPLOS-2017,txm:ReDU:Micro-2018,arch:Dolos-secure:Micro-2021}. 

\subsubsection{Throughput}\ 

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{./pic/eval/mi1tp.pdf}
	\caption{A comparison on transaction throughput of micro-benchmarks (normalized against OPT)}
	\label{fig:micro-txThroughput}
	\vspace{-2ex}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{./pic/eval/mi1writes.pdf}
	\caption{A comparison on pmem writes micro-benchmarks (normalized against OPT)}
	\label{fig:micro-txwrites}
	\vspace{-2ex}
\end{figure*}

We compare \Attend to state-of-the-art hardware designs,
% including Kiln~\cite{txm:Kiln:MICRO13}, TC~\cite{txm:transaction-cache:DAC17}, HOOP~\cite{txm:HOOP:ISCA20}, Proteus~\cite{txm:Proteus:MICRO17}, FWB~\cite{txm:Steal-but-No-Force:HPCA18}, and PiCL~\cite{txm:PiCL:MICRO18}.
including Kiln, TC, HOOP, Proteus, FWB, and PiCL.
They 
represent different
approaches to guarantee atomic durability with pmem %for in-pmem data 
(cf. Section~\ref{sec:bg-ad}).
As PiCL is in a different approach with periodical checkpointing,
we  discuss it separately
in Section~\ref{sec:checkpoint}.
%with non-volatile LLC or side-path cache, hardware undo or redo logging, or both. 
In~\autoref{tab:config}, 
the STT-RAM LLC and side-path cache are for Kiln and TC, respectively,
%is used by Kiln and the side-path STT-RAM cache for TC is set in 4KB \cite{txm:transaction-cache:DAC17},
both configured in line with
%We configure a larger capacity and longer access latency in line with 
%the characteristics of STT-RAM
STT-RAM's characteristics 
\cite{arch:STT-RAM:Micro-2011,txm:Kiln:MICRO13}.
The
software logging with eADR (SWL\_eADR)
is also covered for evaluation while 
the other one without eADR is omitted for brevity.





\input{micro3}
\input{para2}
\input{energy3}
\input{macro2}


==> pd4.tex <==
\subsection{Persistence Domain}

\textbf{Pmem.}\hspace{0.5ex}
Pmem embraces both byte-addressability and persistency. 
Researchers
have considered building pmem with various memory technologies,
such as 
phase-change memory \cite{pmem:PCM:Micro-2009,pmem:PCM:ISCA-2009,pcm:pcm:micro10,arch:PCM-refresh:IEEE-Micro-2011,arch:PCM:HPCA-2011,arch:SD-PCM:ASPLOS-2015,arch:PCM:ISCA-2016},
spin-transfer torque RAM (STT-RAM) \cite{pmem:everspin2,arch:STT-RAM:DAC-2014,txm:checkpoint-SST-RAM:ICCAD-2014,arch:STT-MRAM:ICCAD-2017,arch:STT-MRAM:ICCD-2017,arch:STT-RAM-ECC:TC-2018}, resistive RAM \cite{arch:ReRAM:HPCA-2015,arch:ReRAM:ISCA-2016,arch:ReRAM-endurance:TACO-2018,arch:ReRAM-PIM:ISCA-2019,arch:RRAM-PIM:Micro-2019}, 
3D XPoint~\cite{intel:3dx,pmem:Intel},
and DRAM backed by flash~\cite{pmem:Dell,pmem:HPE,pmem:SMARTM,pmem:Micron,Btree:NV-Tree:FAST-2015}.  
Applications can 
 directly load and store data with pmem
\cite{pmem:Mnemosyne:ASPLOS11,NVM:NVM-Duet:ASPLOS-2014,pmem:NV-Heaps:SIGARCH14,intel:3dx,Btree:NV-Tree:FAST-2015,pmem:DudeTM:SIGARCH17,arch:VANS-LENS:Micro-2020,pmem:Timestone:ASPLOS20,pmem:Optane-study:FAST-2020,arch:stealth-persist:HPCA-2021,pmem:programming:Scargall2020,pmem:survey:acmsurv21,txm:ThyNVM:Micro-2015}.

\textbf{Persistence Domain.}\hspace{0.5ex}
Persistence domain
is  
a region of computer system in which data would not be lost but retrievable %lose
when the system crashes or power failures occur~\cite{pmem:programming:Scargall2020,eADR:Intel}.
It conventionally includes
  disk drives at the secondary storage level.
The advent of pmem brings it up to the memory level.
 

 
\textbf{ADR.}\hspace{0.5ex}
The ADR   
further extends
the persistence domain to the WPQ of 
MC~\cite{arch:eADR:PLDI-2021,txm:LAD:MICRO19,txm:Proteus:MICRO17,arch:Dolos-secure:Micro-2021}.
ADR guarantees that data received at the WPQ can be flushed to pmem upon a %in case of 
power outage.
Though,
the persistence enabled by ADR is transient, as it is the pmem that eventually makes data persistent.
Also,
CPU cache is still volatile  
and cache lines would be lost on a  
crash. 
Thus,
programmers must explicitly flush data staying in cache lines (e.g., \texttt{clwb}) to pmem.
Flushing data from CPU cache to pmem
is not only synchronized and time-consuming, but is also error-prone and hurts programmability~\cite{pmem:programming-is-hard:apsys17,arch:BBB:HPCA-2021}. 

 
\textbf{eADR.}\hspace{0.5ex}	
{Intel extended ADR as eADR which guarantees to 
flush all cache lines 
to pmem in case of a power outage by employing extra power supply} 
\cite{eADR:Intel,pmem:programming:Scargall2020}.
{Alshboul et al.~\cite{arch:BBB:HPCA-2021} proposed BBB that
employs a battery-backed persist buffer alongside each core's L1D cache}
{and achieves an identical effect as eADR with much less cost.} {They help programmers 
avoid explicit cache line flushes.}
More important,
they
 make   
the multi-level CPU cache hierarchy provide
a transient persistence domain in dozens of megabytes
on top of pmem.
 
